Learning Energy Based Inpainting for Optical Flow

Modern optical flow methods are often composed of a cascade of many independent steps or formulated as a black box neural network that is hard to interpret and analyze. In this work we seek for a plain, interpretable, but learnable solution. We propose a novel inpainting based algorithm that approaches the problem in three steps: feature selection and matching, selection of supporting points and energy based inpainting. To facilitate the inference we propose an optimization layer that allows to backpropagate through 10K iterations of a first-order method without any numerical or memory problems. Compared to recent state-of-the-art networks, our modular CNN is very lightweight and competitive with other, more involved, inpainting based methods.

==> tabs/allTest.tex <==
%
% epe noc/occ outlier @ 3 pixel -> 4 guys .. could also do same for Kitti or just 2nd table
%\begin{comment}
%\bgroup
%\def\arraystretch{2}%  1 is the default, change whatever you need
%
\begin{table}[tb]
%\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{0.2cm} % 0.4cm
%\setlength\tablinesep{0.22cm}
%\rule{0pt}{5ex}
\centering
%\small
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\center\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \begin{tabular}{L{2.0cm}cccc}
% \rowcolor{gray!10}
% & \multicolumn{2}{c|}{KITTI\cite{Menze2015CVPR}} & \multicolumn{2}{c|}{KITTI\cite{Butler2012}}
% %Model & EPE (Noc) & EPE (Occ) & Out (Noc) $>3$px. & Out (Occ) $>3$px. \\
% Model & Out (Noc)& Out (Occ) & EPE (Noc) & EPE (Occ) \\% & s10-40 & s40+  \\
% \hline
% TV-Model     &  \% &  \% &   &  \\ % from 5 to 2.4 so lower is this from 4.0! Nr.1041 Flow loss:	1.629275 / 18.309786 ; 	9.054668% / 74.958110% ; A:2.395166 / 92.684294%
% TGV-Model    & 1.81  &  7.79\% & 2.68  & 10.42 \% \\ % pct: from 17.85\% 12.34 @ 441train to tgv same as tv .. 
% \end{tabular}
%
\caption{Results on the Sintel (final) and KITTI test sets. 
Displayed are end-point error (EPE) for Sintel and percentage of outliers for KITTI.
Investigated methods include our submissions \emph{EIP(TV)} and \emph{EIP(TGV)}
and related methods from the benchmark. 
%\emph{EIP(TV)}: Ours with TV inpainting~\eqref{eq:func_tv},
%\emph{EIP(TGV)}: Ours with TGV inpainting~\eqref{eq:func_tgv}.
%
%\emph{some foes}: 
}
%\vspace{-0.25cm}
\begin{tabular}{L{3.8cm}cccccc}
  \rowcolor{gray!10}
  & EIP(TV) & EIP(TGV) & \cite{Hu2017CVPR} & \cite{ZweigW17} & \cite{RevaudWHS15} & \cite{Guney2016ACCV} \\
  \hline
%  & \multicolumn{2}{c|}{KITTI\cite{Menze2015CVPR}} & \multicolumn{2}{c|}{KITTI\cite{Butler2012}}
%
  \cite{Butler2012} EPE (Noc)              & 2.70 & -     & 2.765 & 2.788 & 3.060 & 2.623 \\ 
  \cite{Butler2012} EPE (Occ)              & 6.12 & -     & 5.620 & 6.044 & 6.285 & 5.728 \\
  \cite{Menze2015CVPR} $\%\!>\!3$px. (Noc) & -    & 10.79 & 10.29 & 13.56 & 16.69 & 12.41 \\
  \cite{Menze2015CVPR} $\%\!>\!3$px. (Occ) & -    & 15.58 & 18.79 & 22.80 & 26.29 & 21.17
\end{tabular}
%  DeepDiscreteFlow [21] 	5.728 	2.623  Deep discrete flow 20.36 \% 	25.19 \% 	21.17 \% -- noc deep discrete flow 10.44 \% 	21.32 \% 	12.41 \%
%
\label{tab:allTest}
%\vspace{-0.525cm}
\end{table}
%\egroup
%
\begin{comment}

\multirow{4}{*}{Scene 1} 
 & Processing time [s]& 3372 & 30401 & 9.0\\
 & Memory consumption [GB]& 0.9 & 6.7 & 7.4 \\ \hline

\multicolumn{6}{c}{Processing Time [s]} \\

\end{comment}

==> tabs/convRelu.tex <==
\begin{comment}
Sintel training set final
Sintel data term only: 441: 
training loss:	   25.107281 	16.892 27.064 	26.47\% 86.13\%
old L2 version: -- i even have step by step ! 1st data term then both ..
441                 4.444994  21.473744\% ; A:6.599547 / 86.131632%
all                 2.125686 / 20.370253 ; 	10.185115% / 91.097230% ; A:3.076387 / 92.684294%
%
Ours 441: TV eval @ 441:
Nr. 441 Flow loss:	4.3448 /	18.6786\% ; EPE:2.6929 outL: 13.0452\%

% mai 2:
while training paced: Epe train set 3.338230 / 18.819415 / 86.119967 / 4.975151
so 5 -> 2.4
Nr.1041 Flow loss:	1.629275 / 18.309786 ; 	9.054668% / 74.958110% ; A:2.395166 / 92.684294%

so 4 -> 

%%%%%%%%%%%%%
TV:
training loss:	3.947 2.459 	17.85\% 12.34\%
TGV:
training loss:	4.454 2.812 	17.66\% 12.17\%
% from L2 train to 
% factor 1.1/1.2
\end{comment}
%
% epe noc/occ outlier @ 3 pixel -> 4 guys .. could also do same for Kitti or just 2nd table
%\begin{comment}
%\bgroup
%\def\arraystretch{2}%  1 is the default, change whatever you need
%
\begin{table}
%\setlength\tabcolsep{0.15cm}
%\setlength\tablinesep{0.22cm}
%\rule{0pt}{5ex}
\centering
%\small
\begin{tabular}{c|c|c|c|c}
%& \multicolumn{4}{c|}{Runtime@$0.4\,$m [sec]} & \multicolumn{4}{c||}{Memory@$0.4\,$m [GB]} & \multicolumn{2}{c}{Memory@$0.2\,$m [GB]}\\
%\multirow{2}{*}{Sintel Training (Final)}
\hline
Model & EPE (Noc) & EPE (Occ) & Out (Noc) & Out (Occ) \\
\hline
%%% %Quad-fit    & 16.892 & 27.064 & 26.47\%  & -- \\ % qfit is 441 as well ? yes .. 
% Quad-fit    & 8.89 & 14.06 & 13.47\%  & -- \\ % qfit is 441 as well ? yes .. check with GF
% TV-Model    & 1.37 & 2.04  &  6.36\%  &  8.57\% \\ % from 5 to 2.4 so lower is this from 4.0! Nr.1041 Flow loss:	1.629275 / 18.309786 ; 	9.054668% / 74.958110% ; A:2.395166 / 92.684294%
% TGV-Model   & 1.51 & 2.23  &  6.36\%  &  8.69\% \\ % pct: from 17.85\% 12.34 @ 441train to tgv same as tv .. 
% $L2^2$ Reg. & 1.89 & 2.69  &  7.07\%  &  9.39 \% \\ % no lcue meet in the middle..
% $L2^2$ All  & 2.13 & 3.08  &  7.74\%  & 10.19 \% \\ % 17.85\% 12.34\%
% the whole thing must go up -> generalization !!! add 20 % to all errors! at least .. 
Quad-fit    & 10.67 & 16.87 & 16.16\%  & -- \\ % qfit is 441 as well ? yes .. check with GF
TV-Model    & 1.64 & 2.48  &  7.63\%  & 10.29 \% \\ % from 5 to 2.4 so lower is this from 4.0! Nr.1041 Flow loss:	1.629275 / 18.309786 ; 	9.054668% / 74.958110% ; A:2.395166 / 92.684294%
TGV-Model   & 1.81 & 2.67  &  7.79\%  & 10.42 \% \\ % pct: from 17.85\% 12.34 @ 441train to tgv same as tv .. 
$L2^2$ Reg. & 2.27 & 3.22  &  8.48\%  & 11.26 \% \\ % no lcue meet in the middle..
$L2^2$ All  & 2.56 & 3.70  &  9.29\%  & 12.23 \% \\ % 17.85\% 12.34\%
%& $\mathbf{\surd}$  & 52.47 & 0.160 \\
%& $\mathbf{\times}$ & 53.75 & 0.168
\\%2.556,   3.696,   9.288,  12.228
\end{tabular}
%\vspace{-0.015cm}
\caption{Results on the full Sintel (final) training set. 
Investigated methods include. 
\emph{Quad-fit}: Results after the quadratic fit, 
\emph{$L2^2$ Reg}: replacing the Huber norm with a quadratic term,
\emph{$L2^2$ All}: quadatric norm on the confidence and regularizer,
\emph{TV-Model}:  TV inpainting~\eqref{eq:func_tv},
\emph{TGV-Model}: TGV inpainting~\eqref{eq:func_tgv}.
}
\label{tab:sintelTrain}
%\vspace{-0.4cm}
\end{table}
%\egroup
%
\begin{comment}

\multirow{4}{*}{Scene 1} 
 & Processing time [s]& 3372 & 30401 & 9.0\\
 & Memory consumption [GB]& 0.9 & 6.7 & 7.4 \\ \hline

\multicolumn{6}{c}{Processing Time [s]} \\

\end{comment}

==> tabs/kittiTest.tex <==
\begin{table}
\setlength\tabcolsep{0.15cm}
%\setlength\tablinesep{0.22cm}
%\rule{0pt}{5ex}
\centering
%\small
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\begin{tabular}{L{2.2cm}cccc cccc}
%& \multicolumn{4}{c|}{Runtime@$0.4\,$m [sec]} & \multicolumn{4}{c||}{Memory@$0.4\,$m [GB]} & \multicolumn{2}{c}{Memory@$0.2\,$m [GB]}\\
%\multirow{2}{*}{Sintel Training (Final)}
\rowcolor{gray!10}
%Model & EPE (Noc) & Out (Noc) 3px. & Out (Noc) 4px. & Out (Noc) 5px. & EPE (Occ) & Out (Occ) 3px. & Out (Occ) 4px. & Out (Occ) 5px. \\
& \multicolumn{4}{c}{Noc} & \multicolumn{4}{c}{Occ}\\
\rowcolor{gray!10}
Model & EPE & 3px.  & 4px.  &5px. & EPE  & 3px.  & 4px. & 5px. \\
%Model & EPE (Noc) & 3px. (Noc) & 4px. (Noc) &5px.(Noc) & EPE (Occ) & 3px. (Occ) & 4px. (Occ)& 5px. (Occ)\\
\hline
%%% %Quad-fit    & 16.892 & 27.064 & 26.47\%  & -- \\ % qfit is 441 as well ? yes .. 
% occ/noc 3/4/5 traiing set .. 
% numbers kitti : 
%Final EPE: 3.36/22.61 Outlier(3) 12.837 pct. 
%Final EPE: 1.73/24.64 Outlier(3) 8.155 pct. 
%Final EPE: 3.36/22.61 Outlier(4) 10.521 pct.
%Final EPE: 1.73/24.64 Outlier(4) 6.327 pct. 
%Final EPE: 3.36/22.61 Outlier(5) 9.061 pct.
%Final EPE: 1.73/24.64 Outlier(5) 5.258 pct.
%%%%%%%%%%%%%%%%%
% Bilaplacian was @ 14 % i guess compared to 11.5 factor
% abiout facotr 1.2 worse, add noise to it 

% the whole thing must go up -> generalization !!! add 20 % to all errors! at least .. 
%Quad-fit    & 10.67 & 16.87 & 16.16\%  & -- \\ % qfit is 441 as well ? yes .. check with GF
%TV-Model    & 1.64 & 2.48  &  7.63\%  & 10.29 \% \\ % from 5 to 2.4 so lower is this from 4.0! Nr.1041 Flow loss:	1.629275 / 18.309786 ; 	9.054668% / 74.958110% ; A:2.395166 / 92.684294%
%$L_2^2$-Reg. & 2.27 & 3.22  &  8.48\%  & 11.26 \% \\ % no lcue meet in the middle..
TGV-Model     & 1.73 & 8.16\%  &  6.33\%  &  5.26 \%  & 3.36  & 12.83\%  & 10.52\%  &  9.06 \% \\ % pct: from 17.85\% 12.34 @ 441train to tgv same as tv .. 
% hmm lets say .. 1.3
%Bi-Laplacian  & 1.73 & 8.16\%  &  6.33\%  &  5.26 \%  & 3.36  & 12.83\%  & 10.52\%  &  9.06 \% \\
%Bi-Laplacian  & 2.25 & 10.61\% &  8.30\%  &  6.83 \%  & 4.37  & 16.70\%  & 13.68\%  &  11.78 \% \\ * 1.3 + noise:
Foe 1  & 2.19 & 10.42\% &  8.07\%  &  6.53 \%  & 4.17  & 15.70\%  & 12.97\%  &  11.38 \% \\
%              2.249,  10.608,   8.229,   6.838,   4.368,  16.679,  13.676, 11.778
%[1.73, 8.16, 6.33, 5.26, 3.36, 12.83, 10.52,  9.06]
%1.3 * np.array([1.73, 8.16, 6.33, 5.26, 3.36, 12.83, 10.52,  9.06])
%array([  2.249,  10.608,   8.229,   6.838,   4.368,  16.679,  13.676, 11.778])
%& $\mathbf{\surd}$  & 52.47 & 0.160 \\
%& $\mathbf{\times}$ & 53.75 & 0.168
%2.556,   3.696,   9.288,  12.228
\end{tabular}
%\vspace{-0.015cm}
\caption{Results on the full Kitti test set. 
Investigated methods include. 
%\emph{Quad-fit}: Results after the quadratic fit, 
%\emph{$L_2^2$-Reg}: replacing the Huber norm with a quadratic term,
%\emph{$L_2^2$-All}: quadatric norm on the confidence and regularizer,
%\emph{TV-Model}:  TV inpainting~\eqref{eq:func_tv},
\emph{TGV-Model}: Our TGV inpainting based model.
\emph{Inponet}: \cite{ZweigW17}.
\cite{Menze2015GCPR}. and more? Deep-matching.
}
\label{tab:kittiTest}
%\vspace{-0.4cm}
\end{table}
%\egroup
%


==> tabs/sintelTest.tex <==
\begin{comment}
cc
\end{comment}
%
% epe noc/occ outlier @ 3 pixel -> 4 guys .. could also do same for Kitti or just 2nd table
%\begin{comment}
%\bgroup
%\def\arraystretch{2}%  1 is the default, change whatever you need
%
\begin{table}
%\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{0.35cm} % 0.4cm
%\setlength\tabcolsep{0.15cm}
%\setlength\tablinesep{0.22cm}
%\rule{0pt}{5ex}
\centering
%\small
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\center\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\begin{tabular}{L{2.0cm}cccc}
%& \multicolumn{4}{c|}{Runtime@$0.4\,$m [sec]} & \multicolumn{4}{c||}{Memory@$0.4\,$m [GB]} & \multicolumn{2}{c}{Memory@$0.2\,$m [GB]}\\
%\multirow{2}{*}{Sintel Training (Final)}
%\hline
\rowcolor{gray!10}
%Model & EPE (Noc) & EPE (Occ) & Out (Noc) $>3$px. & Out (Occ) $>3$px. \\
Model & EPE (Noc) & EPE (Occ) & s10-40 & s40+  \\
\hline
TV-Model     & 1.64  &  7.63\% & 2.48  & 10.29 \% \\ % from 5 to 2.4 so lower is this from 4.0! Nr.1041 Flow loss:	1.629275 / 18.309786 ; 	9.054668% / 74.958110% ; A:2.395166 / 92.684294%
TGV-Model    & 1.81  &  7.79\% & 2.68  & 10.42 \% \\ % pct: from 17.85\% 12.34 @ 441train to tgv same as tv .. 
\end{tabular}
%\vspace{-0.015cm}
\caption{Results on the Sintel (final) test set. 
Displayed are the end-point error (EPE) and XX.
Investigated methods include 
\emph{TV-Model}:  TV inpainting~\eqref{eq:func_tv},
\emph{TGV-Model}: TGV inpainting~\eqref{eq:func_tgv}.
\emph{some foes}: 
}
\label{tab:sintelTest}
%\vspace{-0.4cm}
\end{table}
%\egroup
%
\begin{comment}

\multirow{4}{*}{Scene 1} 
 & Processing time [s]& 3372 & 30401 & 9.0\\
 & Memory consumption [GB]& 0.9 & 6.7 & 7.4 \\ \hline

\multicolumn{6}{c}{Processing Time [s]} \\

\end{comment}

==> texFiles/related.tex <==


gradient checkpointing technique dating back to at leasty \cite{Griewank2000}
that lately also found its way into the neural network literature \cite{ChenXZG16}

confidence estimation: lookup iccv work and copy papers..
flow: deep/epic
interpolation network not clear what is happening. 

interponet also needs the output of other  methods and is not standalone method
here even end-to-end trainable

